A Missing Information Loss function for implicit feedback datasets

Latent factor models for Recommender Systems with implicit feedback typically treat unobserved user-item interactions (i.e. missing information) as negative feedback. This is frequently done either through negative sampling (point--wise loss) or with a ranking loss function (pair-- or list--wise estimation). Since a zero preference recommendation is a valid solution for most common objective functions, regarding unknown values as actual zeros results in users having a zero preference recommendation for most of the available items. In this paper we propose a novel objective function, the \emph{Missing Information Loss} (MIL), that explicitly forbids treating unobserved user-item interactions as positive or negative feedback. We apply this loss to both traditional Matrix Factorization and user--based Denoising Autoencoder, and compare it with other established objective functions such as cross-entropy (both point- and pair-wise) or the recently proposed multinomial log-likelihood. MIL achieves competitive performance in ranking-aware metrics when applied to three datasets. Furthermore, we show that such a relevance in the recommendation is obtained while displaying popular items less frequently (up to a $20 \%$ decrease with respect to the best competing method). This debiasing from the recommendation of popular items favours the appearance of infrequent items (up to a $50 \%$ increase of long-tail recommendations), a valuable feature for Recommender Systems with a large catalogue of products.

==> conclusions.tex <==
\section{Conclusions and next steps}\label{sec:conclusions}
% definition of MIL
In this paper we present a novel objective function, the \emph{Missing Information Loss} (MIL), specifically designed for handling unobserved user-item interactions in implicit feedback datasets. In particular, MIL explicitly forbids treating missing user-item interactions as positive or negative feedback.
% What it does
We demonstrate that, thanks to the functional form of the MIL function, the ranking of unseen items is almost entirely left to the low--rank process, rather than forcing unobserved items to be at the tail of the recommendation (\emph{i.e.}, MIL does not force a zero predicted preference for unobserved user-item interactions). 

% Metric results
Extensive experiments with Matrix Factorization and Denoising Autoencoders conducted on three datasets, show that \textsc{MIL} models demonstrate competitive performance when compared with other traditional losses such as cross-entropy or the multinomial log-likelihood. 
% Best performing models 
% Analysis of recommendations
In addition, we study the distribution of the recommendations and observe that the reported metric performance takes place while recommending popular items less frequently (up to a $20 \%$ decrease with respect to the best competing method). Indeed, \textsc{MIL} models sharply increase the recommendation of medium--tail items, while almost linearly expanding the appearance of long--tail items with the ranking position in the list of recommendations. Such expansion results in up to a $50 \%$ increase of long--tail recommendations, a feature of utmost importance for industries with a large catalogue of items. 

% Future work
Future lines of research may involve the incorporation of negative feedback, or the usage of \textsc{MIL} in temporal--aware Recommender Systems (such as those using Recurrent Neural Networks).  
In addition, we hope that the results here reported  will bring forward first-principle mathematical derivations of the \textsc{MIL} function, so that the vast family of possible polynomials modelling the missing information term can be reduced, or even extended with more suitable functions. 

==> regularization.tex <==
\subsection{Regularization techniques}\label{subsec:model_regularizations}
In the following, we detail some regularization techniques that are commonly applied to AE, and discuss its usage for RS.
\paragraph{Weight--decay} It is perhaps the most widely used form of regularization in RS. 
% definition of L2
It consists of adding to the loss a Lagrange multiplier with the sum of the Frobenius norm of weight matrices, as biases are typically not regularized,
\begin{equation}\label{eq:L2_reg}
\mathcal{L} = \mathcal{L}_{\rm point/pair}+\frac{1}{2}\lambda\left( ||{\bf W}||_2^2+||{\bf W'}||_2^2\right).
\end{equation}
Here, $\lambda$ is a hyper-parameter. 
The minimization of equation~(\ref{eq:L2_reg}) will tend to make the second term as small as possible~\cite{Goodfellow-et-al-2016}. 
% drawbacks
Nevertheless, there are some drawbacks associated with this type of regularization: (a) the $\lambda$ parameter depends on the natural minimum value of the loss $\mathcal{L}_{\rm point/pair}$, which varies among objective functions and problem types; and (b) it is typically applied with a single hyper-parameter for all weight matrices, even though the scale of each trainable variable might be quite different. This is most critical in matrix factorization algorithms, where the user matrix is defined in $\mathbb{R}^{|\mathcal{U}|\times D}$, while the one for items belongs to $\mathbb{R}^{|\mathcal{I}|\times D}$. Since $|\mathcal{U}|\gg\ |\mathcal{I}|$ in most RS, the user weight matrix is more regularized than its item counterpart. Nevertheless, since we only use the AE architecture along this paper, point (b) is of no concern here. Regarding the variance of $\lambda$ in equation~(\ref{eq:L2_reg}), we will show some examples in section~\ref{sec:results}. 

\paragraph{Max norm} 
% historical perspective
This form of regularization is fairly widespread in the neural networks community, 
after it was discussed by the authors of drop-out in the same paper~\cite{Srivastava:2014:dropout}.
However, it was first introduced in the context of matrix factorization~\cite{Srebro:2005:max_norm}. 
Surprisingly, it is not as adopted in the RS community as it is in the neural networks community.
%max norm definition
Max norm regularization consists in clipping the norm of every item embedding as well as its decoding
(${\bf W}_{:,i}$ and ${\bf W'}_{i,:}$ for $i=1,\ldots , |\mathcal{I}|$) in each training step.
Said clipping ensures that its norm never exceeds a given threshold, while not changing the gradient direction.
In order to apply this regularization with the same strength to all trainable variables, we use the following implementation,
\begin{equation}\label{eq:max_norm_implementation}
{\bf x} = {\bf x}\frac{n}{||{\bf x}||_2}\,\,\, {\rm if}\, ||{\bf x}||_2>n,~~~n^2 = \alpha^2 {\rm dim}({\bf x}),
\end{equation}
with $\alpha$ a hyper-parameter and ${\bf x}\in \{ {\bf W}_{:,i}$,${\bf W'}_{i,:} \}$, for each $i=1,\ldots , |\mathcal{I}|$. In this paper we do not regularize the biases, and use independent regularization strengths for the encoder/decoder, $\alpha_{\rm enc/dec}$.

\paragraph{Noise}
Training neural networks with noise injection is another regularization technique commonly employed within the neural networks community~\cite{Goodfellow-et-al-2016}.
By applying noise, we turn off a subset of neurons in a network, namely, we increase the size of the training set adding to it corrupted examples.
% DAE
When applied to AEs~\cite{Vincent:2008:ECRF-AE}, noise injection prevents learning the identity function as the internal representation of the input.
Instead, it forces a more robust learning procedure that is less sensitive to data fluctuations. Denoising AEs (DAE) are becoming ubiquitous in RS literature, see e.g.~\cite{Wu:2016:CDAE-topN, liang:2018:VAE, Li:2015:DCF_marginalizedAE}.



